Broccoli: Bug localization with the help of text search engines

Bug localization is a tedious activity in the bug fixing process in which a software developer tries to locate bugs in the source code described in a bug report. Since this process is time-consuming and requires additional knowledge about the software project, information retrieval techniques can aid the bug localization process. In this paper, we investigate if normal text search engines can improve existing bug localization approaches. In a case study, we evaluate the performance of our search engine approach Broccoli against seven state-of-the-art bug localization algorithms on 82 open source projects in two data sets. Our results show that including a search engine can increase the performance of the bug localization and that it is a useful extension to existing approaches. As part of our analysis we also exposed a flaw in a commonly used benchmark strategy, i.e., that files of a single release are considered. To increase the number of detectable files, we mitigate this flaw by considering the state of the software repository at the time of the bug report. Our results show that using single releases may lead to an underestimation of the the prediction performance.

==> abstract.tex <==
    Bug localization is a tedious activity in the bug fixing process in which a software developer tries to locate bugs in the source code described in a bug report. Since this process is time-consuming and sometimes requires additional knowledge about the software project, information retrieval techniques can aid the bug localization process. In this paper, we introduce a new bug localization approach, called Broccoli, which uses techniques from previous approaches and extends them with a search engine to improve the localization. In a case study, we evaluate the performance of our search engine approach against seven state-of-the-art bug localization algorithms on 82 open source projects in two data sets. Our results show that including a search engine can increase the performance of the bug localization and that it is a useful extension to existing approaches.
    For the comparison of the bug localization approaches, we use a benchmark strategy commonly used in the community. This strategy, however, only considers files that are contained in a single release. To increase the number of detectable files, we extend this benchmark strategy by considering the state of the software repository at the time of the bug report. Our results show that the previously used benchmark may underestimated the prediction performance, for which our Time-aware strategy provides a better approximation.

==> textCopy.tex <==

In Phase 1, we reused the data set of Bench4BL \cite{lee}. Considering the \gls{MAP} and \gls{MRR} values, the results indicate that none of the bug localization approaches perform significantly better than the others on the data set. Blizzard and BugLocator, however, never achieved the highest \gls{MAP} or \gls{MRR} value on a single project. Therefore, we conclude, that these algorithms should not be selected to perform a bug localization. The other approaches, on the other hand, achieved the highest \gls{MAP} or \gls{MRR} in at least one project. In consideration of all projects, Broccoli has the highest \gls{MRR} and \gls{MAP} value. Further, the discrepancy between the \gls{MRR} and \gls{MAP} values for Locus and BRTracer+ should be considered. Locus has a better \gls{MAP} mean rank then BRTracer, but the \gls{MRR} mean rank of BRTracer+ is better than Locus. However, the literature did not specify, which metric can help a software developer better to locate the buggy file.




In Phase 2, we used the data collected by the SmartSHARK infrastructure \cite{trautsch2020smartshark}. The results demonstrate the power of our search engine approach, since Broccoli has the highest \gls{MAP} value in 16 of 31 projects. The results shows that Broccoli perform significantly better than the other approaches on the data set regarding the \gls{MAP} value. Broccoli was only able to achieve the highest \gls{MRR} value in 4 of 31 projects. BRTracer+ performs best on this data set regarding the \gls{MRR} value. However, the statistical analysis was not able to show the indicated difference between BRTracer+ and Broccoli regarding the \gls{MRR} value.

Considering the statistics of the projects where Broccoli performed worse on the \gls{MRR}, it is apparent that these projects only have few bug reports. The project \emph{commons-digester}, which only contains eight bug reports, is the only project, where Broccoli does not have the best \gls{MRR} value. This result is consistent with the result of the first experiment. These outliers can be explained by insufficient historical data, where approaches using regular expression and simpler heuristics perform better. However, most of the software projects have enough historical data and additionally Broccoli can be adjusted for the projects with less historical data. Another possible solution is to provide the number of bug reports as well as the number of files and commits to the Random Forest algorithm and use this information in order to adjust the components according to the project's statistics. For example, the bug report similarity component can use the number of bug reports to weight its outcome based on the amount of information provided. Alternatively the Random Forest can weight the outcome. 

Moreover, some subjects in the data set can lead to outliers. For example, the JBoss project \emph{WFARQ} only contains one bug report. Thus, if only this bug report is located correctly by the approach, it is likely to produce outliers. This can, for example, be the case if the detection of the algorithm is specialized to the type of the bug report. These outliers can than influence the statistical analysis. For example, BLUiR and AmaLgam reach 1 in the \gls{MAP} and 1 in the \gls{MRR} value on the \emph{WFARQ} project, although the average value and the mean rank is lower. More examples with a low number of bug reports in the data set are \emph{CRYPTO}, \emph{WEAVER}, \emph{WFMP}, \emph{SHL}, \emph{SOCIALLI}, \emph{SOCAILTW}. In four of these seven projects, Broccoli did not attain the best score in the \gls{MAP} value or \gls{MRR} value. A possible reason is that our approach uses data from similar bug reports and the version history to predict the bug location. The short data history of the projects leads to a incorrect prediction. However, it is possible to overcome this issue by retraining the scoring algorithm or collecting more historical data. 


Finally, we identified several issues with the current bug localization benchmarking. Lee et al. \cite{lee}  already proposed a technique called multi version matching to overcome these issues. However, the selection of the correct source code according to a bug report is not completely solved and can be improved even more. Our first experiment on the matching strategy shows that 22.6\% of the files modified in bug reports are not part of the corresponding source code. Moreover, 10.6\% of a bug reports in the SmartSHARK data set contain fixed files that are not predictable, because the source code is not available. Selecting only a single version for each bug report leads to an inaccurate performance evaluation for bug localization approaches. Therefore, we proposed a new strategy, called Time-Aware matching, which allows the selection of multiple source code versions for a single bug report. Table \ref{tab:statistics} shows a comparison between both strategies regarding the detectable files and detectable bug reports. Time-Aware matching is able to increase the number of detectable files and thereby also increases the number of bug reports that are detectable. Therefore, the performance evaluation of the localization can be more accurate, since the algorithm has the chance to detect nearly all bug reports and more files.


All in all our results show a significant difference in 3 of 4 measurements in two independent data sets.  Although we cannot statistically prove the influence of search engines on bug localization in any case, taking into account Figure \ref{fig:featureImportance}, we would like to emphasize that search engines have the ability to increase the performance of bug localization, because they are domain-independent and utilize highly optimized information retrieval techniques that are able to locate the bug more precisely.




Considering the \gls{MAP}, the results indicate that Broccoli performs significantly better than the others on both data set. The performance difference between Broccoli and AmaLgam+, BLUiR+ and Blizzard is significant. The difference between Broccoli and the other approaches is not significant. In the second experiment, the best mean \gls{MRR} was achieved by BRTracer+ followed by Broccoli. However, this difference was not significant. Further, the discrepancy between the \gls{MRR} and \gls{MAP} values could be explained that the search engine generally ranks all files of the search space. Thus, the performance of Broccoli is slightly inferior regarding the \gls{MRR} score. However, the literature did not specify, which metric can help a software developer better to locate the buggy file.
